On the Impact of Gas-Line Absorption in Long-Haul C+L-Band Hollow-Core Fibre Transmission

We numerically investigate gas-line absorption in hollow-core fibre C+L-band transmission. Results show limited C-band but severe L-band performance degradation. Ideal suppression enables a 1.5$\times$ higher L-band throughput, reaching 59.1 Tb/s over 1000 km, while reducing repeater number by up to 3.3$\times$.

==> Figures/throughput_gla_span_2.tex <==
\begin{figure*}
\centering
\begin{tikzpicture}\small
    \begin{groupplot}[
        group style={group size=2 by 1,horizontal sep=40pt,xlabels at=edge bottom},
        grid=both,
        width=.52\linewidth-7.74338/2pt,
        height=6cm,
        ylabel near ticks,
        xlabel near ticks,
        ylabel shift = -2 pt,
        xlabel shift = -2 pt,
        % minor y tick num = 1,
        xlabel={Span length~[km]},
        ylabel={Throughput~[Tb/s]},
        ymin=35,
        ymax=60,
        ytick={35,40,45,50,55,60},
        yticklabels={35,40,45,50,55,60},
        xmin=50,
        xmax=350,
        xtick={50,100,150,200,250,300,350},
        xticklabels={50,100,150,200,250,300,350},
        % title style={at={(0.8,0.96)},font=\bfseries},
        % title style={yshift=-0.5em},
        % label style={font=\small},
    ]
    \newcommand\marksize{1pt}
    \nextgroupplot[
        legend columns=8,
        legend style={fill opacity=1,draw opacity=1,text opacity=1,at={(0.0,1.04)},anchor=south west,draw=black,/tikz/font=\footnotesize},
        legend cell align={left},
        legend image post style={xscale=0.9},
    ]
        \addplot[Set1-A,thick,solid,mark=o,mark size=\marksize,forget plot] table[x=span_length_km,y=P027_gla100] {Data/throughput_L_all_gla_all_power.txt};
        \addplot[Set1-A,thick,dashed,mark=square,mark size=\marksize,forget plot] table[x=span_length_km,y=tp_gla1d00_dattm0d01] {Data/L_throughput_datt.txt};
        \addplot[Set1-A,thick,dotted,mark=triangle,mark size=\marksize,forget plot] table[x=span_length_km,y=tp_gla1d00_dattm0d03] {Data/L_throughput_datt.txt};
        \addplot[Set1-A,thick,dashdotted,mark=diamond,mark size=\marksize,forget plot] table[x=span_length_km,y=tp_gla1d00_dattm0d05] {Data/L_throughput_datt.txt};

        \addplot[Set1-B,thick,solid,mark=o,mark size=\marksize,forget plot] table[x=span_length_km,y=P027_gla040] {Data/throughput_L_all_gla_all_power.txt};
        \addplot[Set1-B,thick,dashed,mark=square,mark size=\marksize,forget plot] table[x=span_length_km,y=tp_gla0d40_dattm0d01] {Data/L_throughput_datt.txt};
        \addplot[Set1-B,thick,dotted,mark=triangle,mark size=\marksize,forget plot] table[x=span_length_km,y=tp_gla0d40_dattm0d03] {Data/L_throughput_datt.txt};
        \addplot[Set1-B,thick,dashdotted,mark=diamond,mark size=\marksize,forget plot] table[x=span_length_km,y=tp_gla0d40_dattm0d05] {Data/L_throughput_datt.txt};

        \addplot[Set1-C,thick,solid,mark=*,mark size=\marksize,forget plot] table[x=span_length_km,y=P027_gla000] {Data/throughput_L_all_gla_all_power.txt};
        \addplot[Set1-C,thick,dashed,mark=square*,mark size=\marksize,forget plot] table[x=span_length_km,y=tp_gla0d00_dattm0d01] {Data/L_throughput_datt.txt};
        \addplot[Set1-C,thick,dotted,mark=triangle*,mark size=\marksize,forget plot] table[x=span_length_km,y=tp_gla0d00_dattm0d03] {Data/L_throughput_datt.txt};
        \addplot[Set1-C,thick,dashdotted,mark=diamond*,mark size=\marksize,forget plot] table[x=span_length_km,y=tp_gla0d00_dattm0d05] {Data/L_throughput_datt.txt};

        \addplot[Set1-D,thick,solid,mark=pentagon*,mark size=\marksize,forget plot] table[x=span,y=l] {Data/throughput_smf.txt};

        \addlegendimage{Set1-D,thick,solid,mark=pentagon*,mark size=\marksize};
        \addlegendentry{SMF};
        \addlegendimage{Set1-A,thick,solid,mark=none};
        \addlegendentry{100\% $p$CO\textsubscript{2}};
        \addlegendimage{Set1-B,thick,solid,mark=none};
        \addlegendentry{40\% $p$CO\textsubscript{2}};
        \addlegendimage{Set1-C,thick,solid,mark=none};
        \addlegendentry{0\% $p$CO\textsubscript{2}};
        \addlegendimage{black,thick,solid,mark=*,mark size=\marksize};
        \addlegendentry{27~dBm};
        \addlegendimage{black,thick,dashed,mark=square*,mark size=\marksize};
        \addlegendentry{32~dBm};
        \addlegendimage{black,thick,dotted,mark=triangle*,mark size=\marksize};
        \addlegendentry{36~dBm};
        \addlegendimage{black,thick,dashdotted,mark=diamond*,mark size=\marksize};
        \addlegendentry{40~dBm};

        \draw [stealth-stealth,thick] (axis cs:100,42.2)--(axis cs:270,42.2) node[midway,fill opacity=0,text opacity=1,inner ysep=2pt,font=\footnotesize,anchor=north] {2.7$\times$};

        % \draw [solid,thick] (axis cs:100,40.2)--(axis cs:100+10,40.2);
        % \draw [solid,thick] (axis cs:100,59.1)--(axis cs:100+10,59.1);
        \draw [stealth-stealth,thick] (axis cs:90,46.9)--(axis cs:90,52.0) node[above,fill opacity=0,text opacity=1,inner ysep=2pt,font=\footnotesize,anchor=south] {5.0~Tb/s};

        \node[anchor=south west,font=\footnotesize] at (rel axis cs:0.01,0.01) {(a)};

    \nextgroupplot[
        legend columns=1,
        legend style={fill opacity=1,draw opacity=1,text opacity=1,at={(0.0,0.0)},anchor=south west,draw=black,/tikz/font=\footnotesize},
        legend cell align={left},
    ]
        \addplot[Set1-A,thick,solid,mark=o,mark size=\marksize,forget plot] table[x=span_length_km,y=P027_gla100] {Data/throughput_L_all_gla_all_power.txt};
        \addplot[Set1-A,thick,dashed,mark=square,mark size=\marksize,forget plot] table[x=span_length_km,y=P032_gla100] {Data/throughput_L_all_gla_all_power.txt};
        \addplot[Set1-A,thick,dotted,mark=triangle,mark size=\marksize,forget plot] table[x=span_length_km,y=P036_gla100] {Data/throughput_L_all_gla_all_power.txt};
        \addplot[Set1-A,thick,dashdotted,mark=diamond,mark size=\marksize,forget plot] table[x=span_length_km,y=P040_gla100] {Data/throughput_L_all_gla_all_power.txt};

        \addplot[Set1-B,thick,solid,mark=o,mark size=\marksize,forget plot] table[x=span_length_km,y=P027_gla040] {Data/throughput_L_all_gla_all_power.txt};
        \addplot[Set1-B,thick,dashed,mark=square,mark size=\marksize,forget plot] table[x=span_length_km,y=P032_gla040] {Data/throughput_L_all_gla_all_power.txt};
        \addplot[Set1-B,thick,dotted,mark=triangle,mark size=\marksize,forget plot] table[x=span_length_km,y=P036_gla040] {Data/throughput_L_all_gla_all_power.txt};
        \addplot[Set1-B,thick,dashdotted,mark=diamond,mark size=\marksize,forget plot] table[x=span_length_km,y=P040_gla040] {Data/throughput_L_all_gla_all_power.txt};

        \addplot[Set1-C,thick,solid,mark=*,mark size=\marksize,forget plot] table[x=span_length_km,y=P027_gla000] {Data/throughput_L_all_gla_all_power.txt};
        \addplot[Set1-C,thick,dashed,mark=square*,mark size=\marksize,forget plot] table[x=span_length_km,y=P032_gla000] {Data/throughput_L_all_gla_all_power.txt};
        \addplot[Set1-C,thick,dotted,mark=triangle*,mark size=\marksize,forget plot] table[x=span_length_km,y=P036_gla000] {Data/throughput_L_all_gla_all_power.txt};
        \addplot[Set1-C,thick,dashdotted,mark=diamond*,mark size=\marksize,forget plot] table[x=span_length_km,y=P040_gla000] {Data/throughput_L_all_gla_all_power.txt};

        \addplot[Set1-D,thick,solid,mark=pentagon*,mark size=\marksize,forget plot] table[x=span,y=l] {Data/throughput_smf.txt};

        % \draw [solid,thick] (axis cs:100,40.2)--(axis cs:100+10,40.2);
        % \draw [solid,thick] (axis cs:100,59.1)--(axis cs:100+10,59.1);
        \draw [stealth-stealth,thick] (axis cs:60,40.2)--(axis cs:60,59.1) node[midway,fill opacity=0,text opacity=1,inner xsep=1pt,font=\footnotesize,anchor=west] {1.5$\times$};

        % \draw [solid,thick] (axis cs:100,56.5)--(axis cs:100,58.5);
        % \draw [solid,thick] (axis cs:333,56.5)--(axis cs:333,58.5);
        % \draw [stealth-stealth,thick] (axis cs:50,55.8)--(axis cs:166.6,55.8) node[midway,fill opacity=0,text opacity=1,inner ysep=2pt,font=\footnotesize,anchor=north] {3.3$\times$};

        % \draw [solid,thick] (axis cs:100,45.5)--(axis cs:100,47.5);
        % \draw [solid,thick] (axis cs:333,45.5)--(axis cs:333,47.5);
        \draw [stealth-stealth,thick] (axis cs:100,48)--(axis cs:333,48) node[midway,fill opacity=0,text opacity=1,inner ysep=2pt,font=\footnotesize,anchor=south] {3.3$\times$};

        \draw [-stealth,thick,rotate=0] (axis cs:200,38.5) arc [start angle=-150,end angle=150,x radius=0.1cm,y radius=0.25cm] node[near start,fill opacity=0,text opacity=1,inner ysep=2pt,font=\footnotesize,anchor=north] {Higher power};
        
        \node[anchor=south west,font=\footnotesize] at (rel axis cs:0.01,0.01) {(b)};

    \end{groupplot}
    
\end{tikzpicture}

\caption{Achieved throughput from (a) C- and (b) L-band 1000~km SMF and HCF transmission with different residual gas conditions, total launch power and span length.}
\label{fig:throughput_gla_span}

\end{figure*}
